Self-supervised Learning on Graphs: Contrastive, Generative,or Predictive

Deep learning on graphs has recently achieved remarkable success on a variety of tasks, while such success relies heavily on the massive and carefully labeled data. However, precise annotations are generally very expensive and time-consuming. To address this problem, self-supervised learning (SSL) is emerging as a new paradigm for extracting informative knowledge through well-designed pretext tasks without relying on manual labels. In this survey, we extend the concept of SSL, which first emerged in the fields of computer vision and natural language processing, to present a timely and comprehensive review of existing SSL techniques for graph data. Specifically, we divide existing graph SSL methods into three categories: contrastive, generative, and predictive. More importantly, unlike other surveys that only provide a high-level description of published research, we present an additional mathematical summary of existing works in a unified framework. Furthermore, to facilitate methodological development and empirical comparisons, we also summarize the commonly used datasets, evaluation metrics, downstream tasks, open-source implementations, and experimental study of various algorithms. Finally, we discuss the technical challenges and potential future directions for improving graph self-supervised learning. Latest advances in graph SSL are summarized in a GitHub repository https://github.com/LirongWu/awesome-graph-self-supervised-learning.

==> tab2_method.tex <==
\begin{table*}[!htbp]
\caption{A summary of the surveyed papers. The classification is organized based on the underlying motivation behind pretext task design.}
\label{tab2:methods}
\centering
\vspace{-1em}
\begin{tabular}{lcccccl}

\hline
\multicolumn{1}{c}{Methods} & \multicolumn{1}{c}{Graph Property} & \multicolumn{1}{c}{Pretext Task} & \multicolumn{1}{c}{Data Augmentation} & \multicolumn{1}{c}{Objective Function} &\multicolumn{1}{c}{Training Strategy} &  \multicolumn{1}{c}{Year} \\ 
\hline

Graph Completion \cite{you2020does} & Attributed & Generative/AE & Attribute Masking & MAE & P\&F/JL & 2020 \\ \hline
GPT-GNN \cite{hu2020gpt} & Heterogeneous & Generative/AR & \tabincell{c}{Attribute Masking \\ Edge Perturbation} & MAE/InfoNCE & P\&F & 2020 \\ \hline

GraphCL \cite{you2020graph} & Attributed & Contrastive/G-G & \tabincell{c}{Attribute Masking \\ Edge Perturbation \\ Random Walk Sampling} & InfoNCE & URL & 2020 \\ \hline
GCC \cite{qiu2020gcc} & Unattributed & Contrastive/C-C & Random Walk Sampling & InfoNCE & P\&F/URL & 2020 \\ \hline
GRACE \cite{zhu2020deep} & Attributed & Contrastive/L-L & \tabincell{c}{Attribute Masking \\ Edge Perturbation} & InfoNCE & URL & 2020 \\ \hline
DGI \cite{velickovic2019deep} & Attributed & Contrastive/L-G & Arbitrary & JS Estimator & URL & 2019 \\ \hline
Subg-Con \cite{jiao2020sub} & Attributed & Contrastive/L-C & Importance Sampling & Triplet Margin & URL & 2020 \\ \hline
SUGAR \cite{sun2021sugar} & Attributed & Contrastive/C-G & BFS Sampling & JS Estimator & JL & 2021 \\ \hline

\tabincell{l}{Node Property \\ Prediction \cite{jin2020self}} & Attributed & Predictive/NP & None & MAE & P\&F/JL & 2020 \\ \hline
Meta-path prediction \cite{hwang2020self} & Heterogeneous & Predictive/CP & None & CE & JL & 2020 \\ \hline
\tabincell{l}{Graph-level \\ Motif Prediction \cite{rong2020self}} & Attributed & Predictive/DK & None & CE & P\&F & 2020 \\ \hline
M3S \cite{sun2020multi} & Attributed & Predictive/ST & None & Clustering & JL & 2020 \\ \hline

\end{tabular}
\vspace{-1em}
\end{table*}


==> tab3_task.tex <==
\begin{table*}[!htbp]
\caption{A summary of implementation details about the surveyed papers, including downstream task level, evaluation metric, and dataset.}
\label{tab3:task}
\centering
\vspace{-1em}
\begin{tabular}{llll}

\hline
\multicolumn{1}{c}{Methods} & \multicolumn{1}{c}{Task Level} &
\multicolumn{1}{c}{Evaluation Metric} & \multicolumn{1}{c}{Dataset} \\ 
\hline

Graph Completion \cite{you2020does} & Node & Node Classification (Acc) & Cora, Citeseer, Pubmed \\ \hline
GPT-GNN \cite{hu2020gpt} & Node/Link & \tabincell{l}{Node Classification (F1-score), \\ Link Prediction (ROC-AUC)} & OAG, Amazon, Reddit \\ \hline

GraphCL \cite{you2020graph} & Graph & \tabincell{l}{Graph Classification (Acc, ROC-AUC)} & \tabincell{l}{NCI1, PROTEINS, D\&D, COLLAB, RDT-B, RDT-M5K, \\ GITHUB, MNIST, CIFAR10, MUTAG, IMDB-B, BBBP, \\ Tox21, ToxCast, SIDER, ClinTox, MUV, HIV, BACE, PPI} \\ \hline
GCC \cite{qiu2020gcc} & Node/Graph & \tabincell{l}{Node Classification (Acc), \\ Graph Classification (Acc)} & \tabincell{l}{US-Airport, H-index, COLLAB, IMDB-B, IMDB-M, \\ RDT-B, RDT-M5K} \\ \hline
GRACE \cite{zhu2020deep} & Node & \tabincell{l}{Node Classification (Acc, Micro-F1)} & Cora, Citeseer, Pubmed, DBLP, Reddit, PPI \\ \hline
DGI \cite{velickovic2019deep} & Node & \tabincell{l}{Node Classification (Acc, Micro-F1)} & Cora, Citeseer, Pubmed, Reddit, PPI \\ \hline
Subg-Con \cite{jiao2020sub} & Node & \tabincell{l}{Node Classification (Acc, Micro-F1)} & Cora, Citeseer, Pubmed, PPI, Flickr, Reddit \\ \hline
InfoGraph \cite{sun2019infograph} & Graph & Graph Classification (Acc) & \tabincell{l}{MUTAG, PTC, RDT-B, RDT-M5K, IMDB-B, \\ QM9, IMDB-M} \\ \hline

\tabincell{l}{Node Property \\ Prediction \cite{jin2020self}} & Node & Node Classification (Acc) & Cora, Citeseer, Pubmed \\ \hline
Meta-path prediction \cite{hwang2020self} & Node/Link & \tabincell{l}{Node Classification (F1-score), \\ Link Prediction (ROC-AUC)} & ACM, IMDB, Last-FM, Book-Crossing \\ \hline
\tabincell{l}{Graph-level \\ Motif Prediction \cite{rong2020self}} & Graph & \tabincell{l}{Graph Classification (Acc), \\ Graph Regression (MAE)} & \tabincell{l}{BBBP, SIDER, ClinTox, BACE, Tox21, ToxCast, ESOL, \\ FreeSolv, Lipo, QM7, QM8} \\ \hline
M3S \cite{sun2020multi} & Node & Node Classification (Acc) & Cora, Citeseer, Pubmed \\ \hline

\end{tabular}
\vspace{-1em}
\end{table*}

==> tab4_dataset.tex <==
\begin{table*}[!htbp]
\caption{A summary and statistics of common graph datasets for graph self-supervised learning.}
\label{tab4:datasets}
\centering
\vspace{-1em}
\begin{tabular}{lllllllll}

\hline
\multicolumn{1}{c}{Dataset} & \multicolumn{1}{c}{Category} & \multicolumn{1}{c}{\#Graph} & \multicolumn{1}{c}{\#Node (Avg.)} & \multicolumn{1}{c}{\#Edge (Avg.)} & \multicolumn{1}{c}{\#Feature} & \multicolumn{1}{c}{\#Class} & \multicolumn{1}{c}{Citation} \\ 
\hline

Wiki-CS \cite{mernyei2020wiki} & Citation Network & 1 & 11701 & 216123 & 300 & 10 & \cite{zhu2020graph}, \cite{jovanovic2021towards}, \cite{thakoor2021bootstrapped} \\ \hline
Coauthor-CS \cite{shchur2018pitfalls} & Citation Network & 1 & 18333 & 81894 & 6805 & 15 & \cite{zhu2020graph}, \cite{mavromatis2020graph}, \cite{thakoor2021bootstrapped}, \cite{kefato2021self} \\ \hline

Reddit \cite{hamilton2017inductive} & Social Network & 1 & 232965 & 11606919 & 602 & 41 & \tabincell{l}{\cite{jin2020self}, \cite{hu2020gpt}, \cite{zhu2020deep}, \cite{peng2020graph}, \cite{velickovic2019deep}, \cite{jiao2020sub}, \\ \cite{peng2020self}, \cite{ma2021improving}} \\ \hline
COLLAB \cite{yanardag2015deep} & Social Networks & 5000 & 74.49 & 2457.78 & - & 2 & \cite{you2020graph}, \cite{zhang2020iterative}, \cite{ren2021label}, \cite{qiu2020gcc} \\ \hline

PPI \cite{zitnik2017predicting} & Protein Networks & 24 & 56944 & 818716 & 50 & 121 & \tabincell{l}{\cite{hu2019strategies}, \cite{you2020graph}, \cite{zhu2020deep}, \cite{peng2020graph}, \cite{peng2020graph}, \cite{velickovic2019deep}, \\ \cite{jiao2020sub}, \cite{peng2020self}, \cite{thakoor2021bootstrapped}} \\ \hline
PROTEINS \cite{dobson2003distinguishing} & Protein Networks & 1113 & 39.06 & 72.81 & 4 & 2 & \cite{you2020graph}, \cite{ren2021label}, \cite{zeng2020contrastive}, \cite{sun2021sugar} \\ \hline

MUTAG \cite{debnath1991structure} & Molecule Graphs & 188 & 17.93 & 19.79 & 7 & 2 & \tabincell{l}{\cite{hu2019strategies}, \cite{you2020graph}, \cite{zhang2020iterative}, \cite{ren2021label}, \cite{hassani2020contrastive}, \cite{sun2019infograph}, \\ \cite{sun2021sugar}} \\ \hline
PTC \cite{shervashidze2011weisfeiler} & Molecule Graphs & 344 & 14.29 & 14.69 & 19 & 2 & \tabincell{l}{\cite{zhang2020iterative}, \cite{hassani2020contrastive}, \cite{sun2019infograph}, \cite{wang2021graph}, \cite{gao2021topoter}, \cite{verma2020towards}, \\ \cite{hu2019strategies}, \cite{ren2021label}, \cite{sun2021sugar}} \\ \hline

MNIST \cite{lecun1998gradient} & Others (Image) & - & 70000 & - & 784 & 10 & \cite{you2020graph} \\ \hline
METR-LA \cite{jagadish2014big} & Others (Traffic) & 1 & 207 & 1515 & 2 & - & \cite{opolka2019spatio} \\ \hline
Amazon-Photo \cite{shchur2018pitfalls} & Others (Purchase) & 1 & 7650 & 119081 & 745 & 8 & \tabincell{l}{\cite{zhu2020graph}, \cite{jovanovic2021towards}, \cite{mavromatis2020graph}, \cite{hu2020gpt}, \cite{thakoor2021bootstrapped}, \cite{jing2021hdmi}, \\ \cite{ma2021improving}, \cite{kefato2021self}} \\ \hline

\end{tabular}
\vspace{-1em}
\end{table*}



==> tab5_github.tex <==
\begin{table}[!htbp]
\caption{A summary of open-source codes of the surveyed papers.}
\label{tab5:github}
\centering
\vspace{-1em}
\begin{tabular}{ll}

\hline
\multicolumn{1}{c}{Methods} & \multicolumn{1}{c}{Github} \\ 
\hline

\tabincell{l}{Graph \\ Completion \cite{you2020does}} & \url{https:
//github.com/Shen-Lab/SS-GCNs} \\ \hline
GPT-GNN \cite{hu2020gpt} & \url{https://github.com/acbull/GPT-GNN} \\ \hline

GraphCL \cite{you2020graph} & \url{https://github.com/Shen-Lab/GraphCL} \\ \hline
GCC \cite{qiu2020gcc} & \url{https://github.com/THUDM/GCC} \\ \hline
GRACE \cite{zhu2020deep} & \url{https://github.com/CRIPAC-DIG/GRACE} \\ \hline
DGI \cite{velickovic2019deep} & \url{https://github.com/PetarV-/DGI} \\ \hline
Subg-Con \cite{jiao2020sub} & \url{https://github.com/yzjiao/Subg-Con} \\ \hline
InfoGraph \cite{sun2019infograph} & \url{https://github.com/fanyun-sun/InfoGraph} \\ \hline

\tabincell{l}{Node Property \\ Prediction \cite{jin2020self}}  & \tabincell{l}{\url{https://github.com/ChandlerBang/Self} \\ \url{Task-GNN}} \\ \hline
\tabincell{l}{Meta-path \\ prediction \cite{hwang2020self}} & \url{https://github.com/mlvlab/SELAR} \\ \hline
\tabincell{l}{Graph-level Motif \\ Prediction \cite{rong2020self}} & \url{https://github.com/tencent-ailab/grover} \\ \hline
M3S \cite{sun2020multi} & \url{https://github.com/datake/M3S} \\ \hline

\end{tabular}
\vspace{-1em}
\end{table}

